Feedback Control Goes Wireless: Guaranteed Stability over Low-power Multi-hop Networks

Closing feedback loops fast and over long distances is key to emerging applications; for example, robot motion control and swarm coordination require update intervals of tens of milliseconds. Low-power wireless technology is preferred for its low cost, small form factor, and flexibility, especially if the devices support multi-hop communication. So far, however, feedback control over wireless multi-hop networks has only been shown for update intervals on the order of seconds. This paper presents a wireless embedded system that tames imperfections impairing control performance (e.g., jitter and message loss), and a control design that exploits the essential properties of this system to provably guarantee closed-loop stability for physical processes with linear time-invariant dynamics. Using experiments on a cyber-physical testbed with 20 wireless nodes and multiple cart-pole systems, we are the first to demonstrate and evaluate feedback control and coordination over wireless multi-hop networks for update intervals of 20 to 50 milliseconds.

==> img/glossySyncError.tex <==
% !TEX root = ../paper.tex
\begin{figure}[!tb]
\centering
\includegraphics[width=\linewidth]{all_absolute_errors2.pdf}
% \vsquish{-7mm}
\caption{Synchronization error of our Glossy implementation for a network diameter of up to nine hops.
%\capt{The error is typically below 1.5\us. The long tail on both sides is due to a race condition in an interrupt service routine.}
}
% \vsquish{-0mm}
\label{fig:eREF_bounds}
\end{figure}


==> problem.tex <==
% !TEX root = paper.tex

%\section{Problem and Related Work}
\section{Problem and Background}
\label{sec:background}
\st{For me: emphasize somewhere that control and process can be spatially distributed / on different nodes.}
Guaranteeing stability for fast closed-loop control over multi-hop low-power wireless networks is an unsolved problem.
%The problem originates from the requirements of current and future \cps applications.
This section provides a brief background on closed-loop control for networked and distributed systems, and formulates the particular challenges that arise when communication is over wireless networks as is envisioned for future cyber-physical system (\cps) applications. % alternative: operation(s)

A \cps is characterized by multiple
%spatially distributed
physical processes interfacing embedded systems, which, in turn, are interconnected over communication networks.
In contrast to pure sensing applications \st{Some references here?  @Marco: Maybe you can add some from low-power wireless, eg. previous applications of LWB?!}\db{Otherwise, \cite{akyildiz2002survey} might be a good ref}, we are interested in \cps that involve sensing \emph{and} actuation.
That is, we address closed-loop control, where sensor data is transformed to actuator commands through control algorithms and an appropriate computing and communication system.
Because introducing \emph{feedback} between sensors and actuators generally modifies the process dynamics, guaranteeing closed-loop stability is a major concern in the design of any control system \cite{Astrom2008}.
%, especially in safety-critical applications.

While control computations are performed on multiple individual devices, coordination among these is vital for realizing most envisioned \cps applications.\fm{"Most envisioned CPS application" is maybe a bit too much. I would use "many envisioned..."}
Reasons requiring coordinated control include a common objective (\eg platooning in autonomous driving~\cite{Besselink2016}); dynamic couplings between the physical processes (\eg large-scale process control~\cite{Zhu2002}); and cooperative usage of shared resources (\eg traffic management~\cite{Li2014}).
% they can share resources, as for example multiple vehicles having to pass the same crossover on a road~\cite{Li2014}.

Coordination obviously requires transmission of information between different entities.
This is enabled through the communication infrastructure.  Over the years, control architectures have evolved depending (in part) on the available communication technology \cite{Yang2005,Baillieul2007}, leading to the prospect of wireless control today (cf.\ \figref{fig:historical})\fm{Why and when do we use cf.?}.
In most traditional control systems, sensors and actuators are connected to a \emph{centralized} controller via point-to-point wires (\figref{fig:historical}, left).
While centralized control is beneficial from an information-theoretic point of view (the decision maker has all information), such an architecture is often impractical or infeasible for large-scale systems.
An alternative is decentralized control, where the large-scale system is split into a number of subsystems, each connected to a local controller, but without signal transfer between them~\cite{Yang2005,Lunze2014}.
However, decentralized control can exhibit severe performance limitations and it may not even be possible to stabilize\fm{Stabilize is perhaps too specific here? As far as I understood, stabilization is only one of many control problems. Maybe we can say sth. like "even be possible to sufficiently control..."} a plant this way~\cite{Yang2005}.
To overcome such limitations while retaining the benefits of distributed control computations, communication networks were introduced, firstly in the form of \emph{wired-bus systems}~\cite{Baillieul2007} (\figref{fig:historical}, center).
While such fieldbus systems are very common in automation and control today \cite{Thomesse2005,Trimpe2012},
% Further suitable references, left out for space: Ne07, decotignie2005ethernet
they involve obvious and significant disadvantages compared to wireless with respect to, \eg installation cost, maintenance, and flexibility.\st{I assume that we talk enough about advantages of wireless in the intro, so that this should be clear.  Otherwise, we might have to expand/add a separate paragraph on this.}
Moreover, wired connections are not feasible in many \cps applications such as the above mentioned.
\emph{Wireless control} (\figref{fig:historical}, right) is largely anticipated as the next major breakthrough in distributed automation and control~\cite{Yang2005,Lunze2014,Hespanha2007,Baillieul2007} and will raise \cps to its full potential.\fm{"Raise CPS to its full potential" sounds more like marketing. We also cannot say if this is the full potential. I would rather say "and make use of the potential of CPS."}


\begin{figure}
\centering
\input{Tikz/Historical.tex}
\caption{Schematics of different control architectures, showing multiple systems with sensors (S) and actuators (A) connected to controllers (Ctrl) over point-to-point wires (left), a fieldbus (center), or a wireless network (right).}
\label{fig:historical}
\end{figure}
%\st{\figref{fig:historical}: I like this figure and think that we should keep it!  But I suggest some changes.  1) Have some space between the drawings. 2) consider adding subcaptions or (better?) titles (can be discussed): `Traditional: hardwired, centralized', `Fieldbus distributed control', `Wireless control'. 3) Instead of System/Ctrl 2, make this $m$/$n$, and add some dots between System 1/System nm and Ctrl1/Ctrl n to indicate that we can have several. 4) S/A boxes can possibly be a bit smaller. 5) Figure caption needs to be adjusted and should, for instance, introduced shorthand notation (A, S, Ctrl).}


% Potential paragraph on advantages of wireless for distributed control
\st{We could have such a separate paragraph on advantages of wireless for distributed control here, elaborating a bit on costs, flexibility (other?) advantages.  We could emphasize, for example, that the network makes it easy to exchange information and thus increases the available information for a controller.  I left this out for now, because I expect the advantages of wireless from the application point of view to be clear already from in the intro.}
%
%Wireless NCS offer great advantages over traditional control systems with respect to, \eg installation cost, maintenance, and flexibility.
%
%Notes: Advantages of wireless for distributed/coordinated control:
%\begin{itemize}
%\item should briefly (re)state the general advantages of wireless (ease of installation, reconfiguration, low-power, ....), where we can also reference back to the introduction;
%\item   in addition, it would be good to also mention advantages from the application/control perspective\st{I think that we shouldn't only focus on challenges of wireless from the eprspective of control; there are also advantages of course...} such as making it easy (in principle) to share information, which can be leveraged for better control (check references \cite{Lunze2014,Hespanha2007,Baillieul2007} for this).
%\end{itemize}



Despite their clear advantages, wireless networks also pose significant challenges for the control design (see \eg \cite{Hespanha2007}). These include in particular:
\begin{compactitem}
\item[1)] \textbf{Limited bandwidth.}   Fundamentally, every network link can transport only a finite amount of information per unit of time; and wireless networks typically have more severe constraints on the achievable bandwidth\st{@Marco: Is it ok to say this?}.  Because feedback control requires timely processing and transfer of information, this is critical.  For example, update intervals must be short enough to permit stabilization of an unstable process~\cite{Walsh2002}.  Owing to limited bandwidth, there is also a trade-off between the number of supported participants and key network services, such as the update interval.
%
%   \item \textbf{Update Interval:} If the process we want to control is open-loop unstable, we will not be able to stabilize it if the update interval becomes too large~\cite{Hespanha2007,Lunze2014}.
%  The maximum update interval that can be tolerated is sometimes referred to as \emph{maximum allowable transfer interval} (MATI)~\cite{Walsh2002}.
%  This MATI depends on the dynamics of the system, \ie faster systems demand for shorter update intervals and are thus more challenging for feedback control over wireless.
%\item \textbf{Limited Bandwidth:} If closing the feedback loop over a wireless network, we only have limited bandwidth.
%This means, there is always a tradeoff: If we want to support more participants, the other outlined challenges as delays and packet losses will be more severe.
%If we want to minimize the effect of these challenges, we are usually only able to support few participants.

\item[2)] \textbf{Delay and jitter.}  While in hardwired point-to-point connections, communication delays are typically small enough to be neglected, they cannot be ignored in wireless communication.
What is more, network delays are not constant, but subject to random variations, thus introducing significant jitter.
Significant delays and jitter both can destabilize a feedback system~\cite{Wittenmark1995}.
%
%  \item \textbf{Delays:} With dedicated point-to-point wires, communication delays are small enough to neglect them. If wireless communication networks are used, they become to large too ignore.
%If the delay is too large, the controller will not be able to react to disturbances in time and thus the system might become unstable.
%Delays in wireless networks are also usually time varying (jitter). In classical controller design, a fixed update interval is assumed. While controllers can deal with jitter up to a certain degree~\cite{Cervin2002,Skaf2009}, it can destabilize the system if it becomes too large.

\item[3)] \textbf{Packet loss.}
Owing to the physics of radio transmission and congestion\st{@Marco: Is it ok to say this?  Not sure what to best say here...}, wireless data transmission can fail with some probability.  Because lost packets mean interrupted feedback, this is an obvious issue for feedback control, which must be considered in the control design.  Moreover, the difficulty to properly characterize loss probability distributions in some wireless networks makes a valid analysis and the derivation of strong theoretical guarantees challenging, if not impossible.
%
%\item \textbf{Packet Losses:} As we will evaluate in \secref{sec:eval}, the controller is able to deal with \iid packet losses up to a large drop probability.
%The problem becomes more challenging, if multiple packets are lost in a row.
%This in the end is similar to a long delay, if there is some disturbance while multiple packets are lost the controller will not be able to react to that and the system may become unstable.

\item[4)] \textbf{Information structure.}
\fm{For me it is not really clear what is meant with "information structure". We use this term at some places but I always feel like I don't really got it.} Typical wireless networks enable information transfer between a subset of all network nodes, such as nearest neighbors.  Hence, control has to deal with constrained information structures, which are fundamentally more challenging than centralized structures~\cite{Yang2005}.\st{Check Siljak or Lunze book on information structures} As additional difficulty, the network topology (\ie the information architecture \fm{What is information architecture? Is it basically the network topology? Since we don't use information architecture later on I would remove this.}) can also vary with time.
%which may, as an additional difficulty, also vary with time.  Which are more challenging than centralized and/or fixed structures.  Such varying and partial information structures
%
%\item \textbf{Information Structure:} Usually the design of a controller is easiest, if we can use a centralised design~\cite{Yang2005}.
%This, however, requires all-to-all communication, what is not necessarily provided by a wireless communication protocol.

\end{compactitem}

If systems and controllers are connected via point-to-point wires, these problems can typically be neglected and are thus not considered in classical control theory~\cite{Hespanha2007,Lunze2014}.
For reliable wireless feedback control, however, they must be addressed.
The faster the physical process being considered, the more pronounced these challenges are.

In this work, we address wireless control for systems that require feedback and control updates at the order of tens of milliseconds.
Closed-loop control at such rates over multi-hop low-power wireless networks has not been achieved before.




%Guaranteeing stability for fast closed-loop control over multi-hop low-power wireless networks is an unsolved problem.
%The problem originates from the requirements of current and future \cps applications.
%This section discusses these requirements and the resulting control and communication challenges, then states the problem we address in this paper, and finally reviews related works.

% ST:
% - Subsection title removed, because there will only be one subsection
% 	(related work to be moved to the end)
% - removed comments that should no be resolved/clear

%\subsection{Application Requirements and Challenges}
%\mz{Initial assignment: Dominik}
%
%\st{I basically started from scratch thinking about what is (in my opinion) a good structure and story for this part...  When you say `application' side, you mean control (possibly combined with the physical application problem), right?  So, I wrote the below outline from this perspective.  While I think I like the outline below and think this section should be rewritten accordingly, please have a look, esp whether this works with the overall paper, and let's discuss.}
%
%\st{In principle, some of the stuff below could also go into the introduction, for which I don't know what is the current plan.  However, to me, it makes sense to talk about the control-related background and challenges in more detail here.  We can, of course, talk about some of this already in the introduction and/or move things around if we prefer so later.}
%
%\st{@Dominik: When you have time, please have a go at this section and we can iterate once I'm back.  However, if there are other things with higher priority, do these first.  Worst case, I should be able to write this up in proper text when I'm back from vacation (as long as we agree on the content now).}

% requirements of current and future \cps applications:
% \begin{compactitem}
%  \item basic structure of a wireless \ncs (see workshop paper): distributed devices, sensors, actuators, controllers, wireless message transfers, tasks (sensing, actuation, control)
%  \item high relevance for different application domains
%  \item need for multi-hop low-power wireless: flexibility (small size, mobile entities), low cost
%  \item particularly interesting for multi-agent systems with many physical systems and many controllers: autonoumous driving, factory automation, quadcopter swarm (see workshop paper)
%  \item linear physical systems are widespread \st{Actually, one can argue that no physical system is actually linear, but linear is a good approximation in many cases. (Don't think we need to go into that much detail though, but just to avoid misunderstanding.)}
% \end{compactitem}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ST: Notes on structure of Section on "Problem and background"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Suggested structure and content:
%\begin{itemize}
%\item The general problem of distributed/coordinated control: physical process(es) with sensing and actuation spatially distributed, need for coordinated feedback control
%\begin{itemize}
%\item Explain why coordination is needed (from the application side); explain on \emph{abstract} level, possibly also mention concrete applications in addition  with references. Reasons for coordination:
%\item (i) dynamic coupling of the physical process
%\item (ii) common objective (\eg formation)
%\item (iii) shared resources (these resources should not be understood as the networked resources, but other `application'-defined resources that must be shared); for example, automatic traffic  management: there is only one crossing and many cars need to go over it, hence, coordination is needed
%\end{itemize}

%\item Historical perspective (brief): How did control and automation deal with the above problem in the past, leading up to wireless network control today\st{I think it makes sense to do it this way, because this naturally introduces wireless control challenges and also gives some background for non control readers.}
%\begin{itemize}
%\item I see three main stages of development (see \cite{Baillieul2007}):
%\item (i) hardwired connections to a centralized controller
%\item (ii) wired bus/fieldbus systems (\cite{Baillieul2007} mentions CAN by Bosch as the first; for general fieldbus systems, this could be refs \cite{Thomesse2005,Ne07} (but double-check))\db{\cite{decotignie2005ethernet}}
%\item (iii) wireless: cite some references that mention wireless networks as the next big step for distributed automation/control (I think \cite{Lunze2014,Hespanha2007,Baillieul2007} all do)
%\item For this historical perspective, we should have some good references here; I looked at these \cite{Lunze2014,Hespanha2007,Baillieul2007}, which I think will do.  @Dominik: If you have additional ones, might want to add.\db{\cite{Yang2005}}
%\item It would be nice (and shouldn't be too difficult, also see \cite[Fig.~1.1]{Lunze2014} for inspiration) to illustrate (i)--(iii) with graphics.
%\end{itemize}

%\item Advantages of wireless for distributed/coordinated control:
%\begin{itemize}
%\item should briefly (re)state the general advantages of wireless (ease of installation, reconfiguration, low-power, ....), where we can also reference back to the introduction;
%\item   in addition, it would be good to also mention advantages from the application/control perspective\st{I think that we shouldn't only focus on challenges of wireless from the eprspective of control; there are also advantages of course...} such as making it easy (in principle) to share information, which can be leveraged for better control (check references \cite{Lunze2014,Hespanha2007,Baillieul2007} for this).
%\end{itemize}

%\item Challenges of wireless for distributed/coordinated control\st{This should obviously match with what we have in the following sections and the overall paper; not sure if I have all.  Also, not sure if the terms that I use are the best ones.}
%\begin{itemize}
%\item I think that we should explicitly list the challenges, enumerate them or so.  And we need to have NCS references that also mention these challenges (again, \cite{Lunze2014,Hespanha2007,Baillieul2007} should be a good start)
%\item 1) Limited bandwidth: From my understanding, this is the update rate of the network, e.g. the rate with which we can transport the data. Here, we can say that especially `fast' systems are a problem\db{also regarding delay especially fast systems are a problem. Drops are a problem if system dynamics are fast compared to sample time. So usually all challenges are harder if we have fast systems\ldots}.
%\db{From my understanding limited bandwidth also contains the number of participants the network can support, not only the update rate.}
%\item 2) Delays: distinguish delay itself and variable delay (jitter); delay itself is a problem, but deterministic is often ok, while variable delay is more problematic (reference here would be good, don't have one now)
%\item 3) Packet dropout: problem in general, but even more if the probability distribution for drops is unknown and/or bursts/non-iid.  Reference some results where stability is lost.
%\item 4) Information structure: By information structure, I mean, who can talk to whom.  Here we can discuss differences between centralized, distributed, decentralized control structures.  Can say that distributed and decentralized is harder than centralized; moreover, can say that variable structures are more difficult (some references needed for this, maybe \cite{Ba08,Si91}, but don't know; Lunze also has a book on this, or course ;)).  (All this leads up to saying later in the paper that all-to-all without changing graphs is great. ;))
%\item OTHER) Are there other challenges, we should mention?  Below, also out-of-order packets are mentioned.  I would try to not go into too many, too detailed challenges here; therefore, maybe out-of-order can also be discussed in the context of 2) above?
%\item To contrast to the traditional control view (see above), we should say that traditionally communication is assumed as ideal (no drop, instantaneous, required bandwidth, etc.; eg \cite{Lunze2014} and \cite[Intro]{Hespanha2007} talk about this).
%\end{itemize}

%\item We can then continue with related work, reviewing what has been done and essentially saying that we are the first to solve the above problems for fast systems.
%\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% First version Dominik
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In \cps, sensing and actuation are often spatially distributed, but they still need a coordinated feedback control.
%Reasons why coordinated control is needed include dynamical couplings of the controlled systems, what is for example the case in certain large-scale process control systems~\cite{Zhu2002}, the systems may follow a common objective, \eg forming a platoon in autonomous driving~\cite{Besselink2016}, or they can share resources, as for example multiple vehicles having to pass the same crossover on a road~\cite{Li2014}.
%
%We want to give an short historic overview, how control dealt with this problem in the past.
%In the beginnings of control, systems were connected with centralized controllers via point-to-point wires~\cite{Yang2005}.
%This is shown in the left part of \figref{fig:historical}\db{I also prepared a figure for a NCS connected over a wired bus. If we want to include this (and maybe coupled dynamics) the figure needs the whole width of the page. As we only wanted to use one page for Sec. 2.1 this might be a bit too much\ldots But inserting it would be no problem, just let me know.}.
%For complex and large-scale systems however, a centralized approach is not feasible.
%Therefore, the large-scale system was split into a number of subsystems, each connected to a local controller, but without signal transfer between different local controllers~\cite{Yang2005,Lunze2014}.
%This so called \emph{decentralized} control without signal transfer between subsystems or local controllers, has severe performance limits and it may not even be possible, to stabilize a plant that way~\cite{Yang2005}.
%In order to transmit information, communication networks were introduced, firstly in the form of wired bus systems~\cite{Baillieul2007}.
%This gave rise to the field of \emph{networked control systems} (NCS).
%Recent developments also allow for the usage of wireless communication networks for distributed control as in the right part of \figref{fig:historical}.
%This is largely anticipated the next breakthrough in the field of distributed automation and control~\cite{Yang2005,Lunze2014,Hespanha2007,Baillieul2007}.
%
%%\begin{figure}
%%\centering
%%\input{Tikz/Historical.tex}
%%\caption{Wired (left) and wireless (right) control system.}
%%\label{fig:historical}
%%\end{figure}
%
%Wireless NCS offer great advantages over traditional control systems with respect to, \eg installation cost, maintenance, and flexibility.
%
%Despite their advantages, they also pose significant challenges for controller design, such as
%\begin{enumerate}
%  \item \textbf{Update Interval:} If the process we want to control is open-loop unstable, we will not be able to stabilize it if the update interval becomes too large~\cite{Hespanha2007,Lunze2014}.
%  The maximum update interval that can be tolerated is sometimes referred to as \emph{maximum allowable transfer interval} (MATI)~\cite{Walsh2002}.
%  This MATI depends on the dynamics of the system, \ie faster systems demand for shorter update intervals and are thus more challenging for feedback control over wireless.
%  \item \textbf{Delays:} With dedicated point-to-point wires, communication delays are small enough to neglect them. If wireless communication networks are used, they become to large too ignore.
%If the delay is too large, the controller will not be able to react to disturbances in time and thus the system might become unstable.
%Delays in wireless networks are also usually time varying (jitter). In classical controller design, a fixed update interval is assumed. While controllers can deal with jitter up to a certain degree~\cite{Cervin2002,Skaf2009}, it can destabilize the system if it becomes too large.
%\item \textbf{Packet Losses:} As we will evaluate in \secref{sec:eval}, the controller is able to deal with \iid packet losses up to a large drop probability.
%The problem becomes more challenging, if multiple packets are lost in a row.
%This in the end is similar to a long delay, if there is some disturbance while multiple packets are lost the controller will not be able to react to that and the system may become unstable.
%\item \textbf{Limited Bandwidth:} If closing the feedback loop over a wireless network, we only have limited bandwidth.
%This means, there is always a tradeoff: If we want to support more participants, the other outlined challenges as delays and packet losses will be more severe.
%If we want to minimize the effect of these challenges, we are usually only able to support few participants.
%\item \textbf{Information Structure:} Usually the design of a controller is easiest, if we can use a centralised design~\cite{Yang2005}.
%This, however, requires all-to-all communication, what is not necessarily provided by a wireless communication protocol.
%\end{enumerate}
%
%If systems and controllers are connected via point-to-point wires, these problems can be neglected and are thus not considered in classical control theory~\cite{Lunze2014}.




% \st{I pretty much ignored the text that is already here and started from scratch when coming up with the above outline, basically thinking about what would work best for this section in my opinion (the purpose of this text in the workshop paper was a bit different).  But, clearly, some of the existing text may be reused.}
% The typical structure of a wireless \cps is shown in \figref{fig:WCS}\st{I think it would be nice if the figure also captured coupled dynamics, e.g. having one physical system with more than one A/S pair.  Also, I think that this drawing can be part of the series of drawings that I mention above in the `history perspective'.}.
% We have multiple physical systems with sensors (S) and actuators (A) that are connected to several controllers over a wireless network.
% The sensors measure some physical quantities of the system and send those measurements over the network to the controllers.
% These controllers then compute actuation commands based on the measurements and send them back over the wireless link to the physical system.
% With the actuation commands the system shall be influenced in a certain way, \eg stabilize it or force it to track a set-point.
% Since multiple feedback loops are closed over the same network, we refer to these kinds of systems as \emph{networked control systems} (NCS)~\cite{Hespanha2007,Lunze2014}.
%
% The concept of NCS is useful for a wide range of applications and different physical systems to be controlled.
% Due to their flexibility and the ease of maintenance NCS are especially interesting for multi-agent scenarios with many systems and many controllers.
% Examples include autonomous driving, where vehicles may communicate to form a platoon; factory automation, where the controller typically resides at some remote location and controls multiple plants; or smart buildings, where sensors and actuators are deployed to regulate the indoor climate.
% As can be seen from these examples, the different physical systems pose varying requirements for the overall NCS.
% The dynamics of the system plays a major role: for example, systems with fast dynamics (\eg mechanical, such as autonomous vehicles) pose more stringent requirements on network communication characteristics than systems with slow dynamics (\eg process plants).
%
% \begin{figure}
% \centering
% \input{Tikz/WirelessFeedbackControl.tex}
% \caption{Typical elements of a wireless \cps. Multiple physical systems with sensors (S) and actuators (A) are connected to multiple controllers over a wireless network.}
% \label{fig:WCS}
% \end{figure}
%
% % challenges to meeting the above requirements:\mz{Add for each challenge what is really the challenge here.}
% % \begin{compactitem}
% %  \item Distributed, decentralized control and coordination
% %  \item Network and system imperfections (see~\cite{Zhang2013})
% %  \begin{itemize}
% %   \item delay
% %   \item jitter
% %   \item packet loss
% %   \item out-of-order message arrivals
% %   \item message duplicates
% %  \end{itemize}
% %  \item Update interval and (end-to-end) delay on the order of tens of milliseconds to keep up with the dynamics of the physical system (\eg mechanical)
% %  \item Resource constraints (energy, bandwidth, compute power, memory) and dynamics of wireless communication
% % \end{compactitem}
%
% Different control architectures and designs are used for NCS depending on, \eg the available sensors, the system size, and the control objectives.
% In principle, a single controller could process data from all sensors and compute commands for all actuators.
% While such a centralized controller has complete information, which is advantageous for control design,
% a centralized approach quickly becomes intractable for large-scale systems (\eg autonomous driving).
% Instead, the control problem may be divided into manageable sub-problems and a decentralized or distributed design be employed, where actuator commands are computed on multiple controllers, \cite{Si91,Ba08}.
% However, owing to the availability of only partial sensor or state information on each individual controller, distributed and decentralized designs are typically more challenging than a centralized design.
%
% While NCS offer great advantages over traditional control systems with respect to, \eg installation cost, maintenance, and flexibility, the communication network does pose significant challenges for control design.
% In classical control, communication is assumed to be perfect: no delay, no jitter, and no packet loss.
% As long as dedicated wired communication links are considered, this assumption may not be too restrictive.
% This changes completely, however, when feedback loops are closed over wireless networks such as in most CPS application scenarios.
%
% \st{This following paragraph contains parts of the solutions (eg predictions, network being iid). IMO, this should generally be  avoided in this part of the paper; here, we should only setup the problem and talk about challenges.  The prposed solutions come later.}
% Delays may partially be compensated by predictions, we will give more details on that in \secref{sec:control}.
% However, if the delay is too large, the controller will not be able to react to disturbances in time and thus the system might become unstable.
% In a similar way, this also holds for packet losses, especially, if they are correlated.
% As we will evaluate in \secref{sec:eval}, the controller is able to deal with \iid packet losses up to a large drop probability.
% The problem becomes more challenging, if multiple packets are lost in a row.
% This in the end is similar to a long delay, if there is some disturbance while multiple packets are lost the controller will not be able to react to that and the system may become unstable.
%
% Design of linear controllers usually assumes that the sampling time is either fast enough to consider it continuous or that it is constant.
% If the sampling time is not constant due to jitter, there are basically two ways to deal with that.
% The controller can be designed in a robust way to be able to deal with differing delays, but this usually decreases performance.
% On the other hand we can also try to spontaneously react to the current sampling time.
% This leads to a more complex controller design and demands some sort of time stamps, to be able to measure the jitter in every round.
%
% If messages arrive out-of-order, this can destabilize the system, as control inputs may be computed based on outdated states of the system.
% When using time stamps or similar, out-of-order packets can be identified and disregarded, this would then be comparable to a longer delay and pose similar challenges as discussed above.
%
% \st{IMO, the content of this paragraph does not belong here. An outline of the contributions and what we will do in this paper, we will (I suppose) give in the introduction.  Approaches like event-/self-triggered, and what is out of the scope of this paper, I don't think need to be mentioned here.  This could be in the concluding remarks/discussion section in the end.}
% In this paper, we want to show, that fast, distributed control and coordination over multi-hop low-power wireless networks is possible.
% Therefore we will show, how we can deal with the above discussed challenged, both from communication and control perspective, give stability guarantees, and evaluate the approach on a physical system.
% Here we will use periodic control and a fixed schedule.
% Event- or self-triggered control schemes as well as schedule adaptations during runtime are also interesting questions in this setting and subject to ongoing research, but are out of the scope of this paper.



% \fakepar{Problem statement}
% Is fast distributed, decentralized control and coordination with stability guarantees for linear systems over multi-hop low-power wireless possible?
%
% out of the scope of this paper:
% \begin{compactitem}
%  \item Event-based or self-triggered control (\ie periodic control)
%  \item Runtime adaptation to changing application requirements (\ie fixed schedule)
% \end{compactitem}


%
%practical work on closed-loop control over wireless:
%\begin{compactitem}
% \item 802.11: \cite{Ye2001} (single-hop, one direction, 12.5\Hz update interval), \cite{Ploplys2004} (single-hop, 2 nodes, both directions, up to 250\Hz update interval, random delays, message loss not considered in control design)
% \item Bluetooth: \cite{Eker2001} (single-hop, 2 nodes, both directions, rotating inverted pendulum, random delays and bit errors, 70\Hz update rate)
% \item 802.15.4: \cite{}
%\end{compactitem}
%
%\cite{Lynch2008}: structural control using semi-active magnetorheological (MR) damper, proprietary 2.4\GHz radio transmitting at 19.2\kbps, single-hop, 4 nodes, only forward direction, 12.5\Hz update rate, LQR control accounting for constant delay but not for message losses
%
%%\fakepar{Networked control}
%
%%\fakepar{Control over (low-power) wireless}
%\cite{Schindler2017}
%\cite{Ceriotti2011}
%\cite{Saifullah2014}
%\cite{Bauer2014}
%
%%\fakepar{Wireless real-time communication}
%
%

%\fakepar{}


%\mz{Initial assignment: Marco}\st{Here, we also need to talk about what has been done on the Control side regarding the above challenges; hopefully Dominik can help with this.  Can be brief though and we can probably reference some of the overviews.}
%
%\cite{verma91,Frehse2014}
%
%\begin{compactitem}
% \item Mainly focus on control over (low-power) wireless $\rightarrow$ use a table (or a figure) comparing our work with existing works along the following dimensions: \#hops, delay/update interval, static/dynamic network, stability proof, $\ldots$
% \item Briefly summarize main efforts on real-time communication in low-power wireless (WirelessHART, ISA 100, Orchestra, TSCH/6TiSCH, Blink, and other works)
%\end{compactitem}

